Good Questions Help Zero-Shot Image Reasoning

Aligning the recent large language models (LLMs) with computer vision models leads to large vision-language models (LVLMs), which have paved the way for zero-shot image reasoning tasks. However, LVLMs are usually trained on short high-level captions only referring to sparse focus regions in images. Such a ``tunnel vision'' limits LVLMs to exploring other relevant contexts in complex scenes. To address this challenge, we introduce Question-Driven Visual Exploration (QVix), a novel prompting strategy that enhances the exploratory capabilities of LVLMs in zero-shot reasoning tasks. QVix leverages LLMs' strong language prior to generate input-exploratory questions with more details than the original query, guiding LVLMs to explore visual content more comprehensively and uncover subtle or peripheral details. QVix enables a wider exploration of visual scenes, improving the LVLMs' reasoning accuracy and depth in tasks such as visual question answering and visual entailment. Our evaluations on various challenging zero-shot vision-language benchmarks, including ScienceQA and fine-grained visual classification, demonstrate that QVix significantly outperforms existing methods, highlighting its effectiveness in bridging the gap between complex visual data and LVLMs' exploratory abilities.

==> sec/4_experiment.tex <==
\section{Experiments}




\begin{table*}[t]
\footnotesize
\centering
    \begin{tabular}{lcccccc}
    \toprule
    \multirow{2}{*}{Method}&\multicolumn{3}{c}{Subject}&\multicolumn{2}{c}{Grade} & \multirow{2}{*}{Average} \\
    \cmidrule(r){2-4} \cmidrule(r){5-6} 
    ~&NAT&SOC&LAN&G1-6&G7-12&~\\
    \midrule
    LLaVA &37.0&61.5 &33.3 &52.3 &30.5 &46.2 \\
    MiniGPT &45.2 &51.5 &38.1 &50.6 & 39.1 &47.4 \\
    InstructBLIP&43.9&58.1&47.6&53.1&39.4&49.3\\  
     \midrule
    QVix (Self-generated question)&47.8&62.9&47.6&58.9&39.4&53.5\\
    QVix (GPT-generated question)&\textbf{48.0}&\textbf{67.1}&\textbf{38.1}&\textbf{60.6}&\textbf{40.5}&\textbf{55.0}\\
    \bottomrule
    \end{tabular}
    \caption{\footnotesize Zero-shot \textbf{visual question-answering (VQA)} accuracy (\%) on ScienceQA. Question categories: NAT = natural science, SOC = social science, LAN = language
science, G1-6 = grades 1-6, G7-12 =
grades 7-12. QVix in the table is applied to InstructBLIP.}
    \label{tab:scienceqa}
       \vspace{-1.5em}
\end{table*}


\begin{table}[htb]
\footnotesize
	\centering
\setlength\tabcolsep{3pt}
    \begin{tabular}{lccc}
    \toprule
    Method&Flowers102&Oxford-IIIT Pet&FGVCAircraft\\
    \midrule
    LLaVA & 36.1 & 39.9 & 15.5 \\
    MiniGPT & 51.5 &63.9 & 14.8\\
    InstructBLIP&59.5&69.8&25.1\\
         \midrule
    QVix (Self-generated) & 66.9 &76.1 & 26.8\\
    QVix (GPT-generated)&\textbf{67.8}&\textbf{80.5}&\textbf{27.7}\\
    \bottomrule
    \end{tabular}
         \caption{\footnotesize Zero-shot \textbf{image classification} accuracy (\%) on Fine-grained Image Classification. QVix is applied to InstructBLIP.}
         \label{tab:imgcls}
            \vspace{-1em}
\end{table}


In this section, we evaluate the proposed QVix in three vision-language tasks: ScienceQA, fine-grained image classification, and Visual Entailment. We show that QVix achieves superior zero-shot performance on these tasks generally compared to other existing baselines. We apply QVix to different LVLMs to show its generality. We conduct a case study to illustrate how QVix attends to important visual areas. Finally, We conduct a thorough analysis of key components of QVix.
\vspace{-1em}
\paragraph{Datasets.} We evaluate our proposal on 5 datasets from three categories of reasoning
tasks: Visual Question Answering, fine-grained image classification and Visual Entailment. For Visual Question Answering, we use ScienceQA~\cite{lu2022learn} which represents a multimodal benchmark encompassing multiple-choice questions across a wide range of scientific subjects. For our evaluation purposes, we exclusively utilized those samples from the test set that are accompanied by images, obtaining a total of 2017 image-question pairs. For fine-grained image classification, we use three popular datasets: Flowers102~\cite{nilsback2008automated}, Oxford-IIIT Pet~\cite{parkhi2012cats} and FGVCAircraft~\cite{maji13fine-grained} which require detailed differentiation of the species of flowers, breeds of pets, and models of cars respectively. For Visual Entailment, we use SNLI-VE which is derived from the Stanford Natural Language Inference (SNLI) initiative by Bowman~\cite{bowman2015large}, which is fundamentally a text entailment (TE) task built upon Flicker30k~\cite{plummer2015flickr30k} data. 
% This framework adapts text entailment to the visual realm, prompting the model to assess if an image semantically aligns with, remains neutral to, or contradicts the given text hypothesis. Consequently, this approach can be viewed as a tripartite classification task. 
In our study, for each dataset, a random selection of 1000 samples was made from the validation/test split. We then assessed our method in a zero-shot context, using accuracy as the metric for evaluation.

\begin{figure}[t]
\vspace{-1.2em}
  \centering
   \includegraphics[width=0.9\linewidth]{figures/hist.pdf}
   \vspace{-1.em}
   \caption{\footnotesize Histograms of the length of the self(VLM)-generated and GPT-generated pre-questions using the prompt in Fig.~\ref{fig:prompt}.}
   \label{fig:hist}
      \vspace{-1.em}
\end{figure}
\vspace{-1em}

\paragraph{Models.} 
We employ two strategies for generating pre-questions. Initially, we tap into GPT~\cite{zhu2023chatgpt} for its advanced reasoning and extensive knowledge, utilizing the 'gpt-3.5-turbo' API for question generation, denoted as ``\textit{GPT-generated questions}''. However, due to the high cost and speed limit of the GPT API, which is impractical for large-scale use, we alternatively generate pre-questions using the embedded LLM in open-source VLMs, greatly increasing our method's usability, denoted as ``\textit{self-generated questions}''. 
For compared baselines, we try three pretrained LVLMs, LLaVA~\cite{liu2023visual}, MiniGPT, and InstructBLIP to do zero-shot reasoning.
\subsection{ScienceQA}

ScienceQA aims to evaluate the model's capacity to navigate and interpret complex scientific information. Each instance in this dataset encompasses a meticulously crafted scientific question, spanning diverse domains including natural science, social science, and language science. 
% Accompanying the question are multiple-choice answers, requiring the model to not only recall scientific facts but also to demonstrate a profound understanding of scientific principles and reasoning. 
The reasoning process of the model may encompass a range of complexities: from straightforward factual queries to intricate problems, understanding of scientific processes, and application of theoretical concepts. 
The performance of various methods on the ScienceQA dataset is examined in Table~\ref{tab:scienceqa}. From Table~\ref{tab:scienceqa}, it's evident that the InstructBLIP method outperforms both LLaVA and MiniGPT in every subject and grade category. Notably, the proposed QVix, whether using self-generated questions or GPT-generated questions,  demonstrates substantial improvement over baselines, particularly in the NAT and SOC subjects, reflecting its strength in generating context-relevant queries. With self-generated questions, QVix achieves a 53.5\% average accuracy, and outperforms the base model InstructBLIP by 4.2\%. When equipped with GPT-generated questions, QVix achieves the highest overall average score of 55.0\%, outperforming that using self-generated questions, which demonstrates that the richer prior knowledge of a more powerful language model can provide better pre-questions. 




\begin{figure*}[htb]
    \footnotesize
  \centering
   \includegraphics[width=1\linewidth]{figures/case.pdf}

   \caption{\footnotesize Case study of QVix and baseline. The attention map is generated by the Q-former of InstructBLIP. }
   \label{fig:case}
   \vspace{-1em}
\end{figure*}

\subsection{Fine-grained Image Classification}

\begin{table}[t]
    \footnotesize
    \centering
    \begin{tabular}{lc}
    \toprule
    Method&Accuracy (\%)\\
    \midrule
    MiniGPT & 35.1 \\
    LLaVA & 40.3  \\
    InstructBLIP&34.5\\
    \midrule
    QVix (Self-generated question) & 43.0 \\
    QVix (GPT-generated question)&\textbf{50.1}\\
    \bottomrule
    \end{tabular}
    \caption{\footnotesize Zero-shot accuracy (\%) on \textbf{Visual Entailment}. QVix in the table is applied to InstructBLIP.}
    \label{tab:ve}
    \vspace{-2em}
\end{table}

\begin{table}[t]
    \footnotesize
    	 \vskip 0.1in
    \centering
    \begin{tabular}{lcc}
    \toprule
    LVLM&Method&Accuracy (\%)\\
    \midrule
    \multirow{2}{*}{MiniGPT}&Baseline & 47.4 \\
    &QVix &\textbf{49.7}\\
    \midrule
    \multirow{2}{*}{Cheetah}&Baseline & 50.0 \\
    &QVix &\textbf{51.9}\\
    \midrule
    \multirow{2}{*}{InstructBLIP}&Baseline & 49.3\\
    &QVix &\textbf{55.0}\\
    \bottomrule
    \end{tabular}
    \caption{\footnotesize Zero-shot VQA accuracy of QVix applied to three LVLMs.}
    \label{tab:generality}
       \vspace{-1em}
\end{table}

Fine-grained Image Classification is a sophisticated task, where the objective is to differentiate between highly similar sub-categories within a broader category. 
% This task is particularly challenging due to the minute differences and high intra-class variation that characterize the categories in question. Excelling in fine-grained image classification often necessitates sophisticated techniques that can recognize and emphasize these subtle, yet critical differences. 
Previous LVLMs performed poorly in fine-grained classification~\cite{xu2023lvlm}. 
% Owing to the large number of categories, typically in the hundreds, it becomes challenging for multimodal large models to process when all categories are presented as input options. Therefore, we first utilize the CLIP~\cite{radford2021learning} model to select the top-5 categories. These categories are then inputted as options for the multimodal large model to facilitate multiple-choice selection.
Table~\ref{tab:imgcls} presents a comparative analysis of different computational methods applied to fine-grained image classification tasks within three specific datasets: Flowers101, Oxford-IIIT Pet, and FGVC-Aircraft. The table highlights the superior performance of our method, QVix, especially when utilizing GPT-generated questions. QVix with GPT-generated questions outshines other methods by achieving the highest accuracy scores across all datasets: 67.8\% for Flowers101, 80.5\% for Oxford-IIIT Pet, and 27.7\% for FGVC-Aircraft. This performance underscores the effectiveness of QVix's strategy of integrating advanced language models to understand and classify images with high granularity.
Comparatively, QVix with self-generated questions also performs robustly, coming in a close second to its GPT-enhanced counterpart, and still outperforms the other listed methods in all datasets. The result indicates that our self-generated questions method is highly competitive, with only a marginal difference when compared to the GPT-generated questions, suggesting that the underlying architecture of QVix is solid even without GPT's assistance.
The success of QVix can be attributed to its ability to generate more contextually relevant  pre-questions that can guide the model to focus on more detail-oriented information within the image that is beneficial for fine-grained classification.
% , a feature that appears to be less pronounced in other methods. For instance, MiniGPT, while showing a substantial gain over LLaVA in all categories, does not reach the performance heights of ArgQue. Similarly, InstructBLIP, despite its commendable results, falls short against ArgQue, particularly in the more challenging Oxford-IIIT Pet and FGVC-Aircraft datasets. In summary, ArgQue demonstrates a significant advantage in fine-grained image classification tasks. The results are indicative of the method's superior ability to process and interpret complex visual information.


\subsection{Visual Entailment}

The task of Visual Entailment involves prompting the model to ascertain if the text is semantically entailed by the image. Each instance contains a coupled set composed of an image and a corresponding text hypothesis, accompanied by three potential answers: entailment, neutral, and contradiction. 
% The model's role is to choose the answer that accurately reflects the interrelation between the image and the text hypothesis. 
Addressing this tri-category classification challenge in a zero-shot framework is notably arduous.
 Table ~\ref{tab:ve} presents a striking demonstration of the effectiveness of our QVix method in the task of Visual Entailment. Significantly, the GPT-generated question variant of QVix achieves an accuracy of 50.1\%, surpassing all other methods by a notable margin. This highlights the advanced understanding and synthesis capabilities of the GPT model when it comes to generating contextually relevant and complex questions for improving visual data understanding, a key component in visual entailment.
Equally important is the performance of QVix with self-generated questions, which records a 43.0\% accuracy. This outstrips the MiniGPT, LLaVA, and InstructBLIP methods by 7.9\%, 2.7\%, and 8.5\%, respectively.
% The relatively lower performance of MiniGPT and InstructBLIP, at 35.1\% and 34.5\% respectively, underscores the challenge that the Visual Entailment task presents to methods using succinct task instruction.  
The success of QVix suggests that the questions with contextual richness and diversity can guide the VLM to comprehensively understand the semantic information of the entire image based on context and details, which is a key demand for Visual Entailment.


\subsection{Analysis}
\label{sec:analysis}
In this subsection, we conduct a thorough analysis of QVix. We show the generality and stability of QVix, perform a case study, and compare QVix with CoT.
In all experiments, we use the test split of ScienceQA, which in our findings is enough to distinguish different model choices.

\vspace{-1em}

\paragraph{Generality of QVix.}
QVix is a general prompting framework that can be applied to different LVLMs. Here we mainly try three different LVLMs: MiniGPT, Cheetah, and InstructBLIP. MiniGPT and InstructBLIP are two highly popular LVLMs, while cheetah is the latest LVLM trained on image-text interleaved data which has strong instruction-following ability. The results are shown in Table~\ref{tab:generality}. 
Across the board, the implementation of QVix results in a consistent improvement in accuracy over the baseline configurations for each of the LVLMs tested. Cheetah, as a state-of-the-art LVLM, demonstrates its robust instruction-following capabilities with a baseline accuracy of 50.0\%. With the integration of QVix, there is a further gain of 1.9\% in accuracy. This increment, while modest, is indicative of QVix's potential to augment even the latest LVLMs that are already optimized for processing complex multimodal data. 
InstructBLIP, another popular LVLM, shows the most significant improvement with QVix, jumping from a baseline accuracy of 49.3\% to 55.0\%.  QVix can serve as a valuable addition to the LVLMs, offering a versatile approach to boosting model performance across a variety of architectures and training paradigms. 

\vspace{-1em}
\paragraph{Case Study.} 
To understand and explain how QVix explores visual information and makes the final reasoning, we provide a case study for baseline and QVix in Fig.~\ref{fig:case}. We visualize the cross-attention map between text and image. Compared to baseline, QVix can attend to important visual areas through those pre-questions. In Sample A, by asking ``\textit{Are there any fallen or collapsed structures in the image?}'', model successfully attends to ``\textit{broken roofs and walls}'' on the ground, which leads to the correct final reasoning. While the baseline only attends to irrelevant areas such as ``\textit{windows}''. Similarly, Sample B's cross-attention maps show QVix's attention to distinctive features of the cat, e.g., ``\textit{eyes}'' and ``\textit{mouse}'', correctly recognizing its breed as Bengal, which is reflective of QVix's ability to parse finer details and patterns in the image. These cases reveal how QVix prompts the model to scrutinize specific visual details that are crucial for accurate image reasoning. This contrasts sharply with the baseline approach, which lacks this directed exploratory mechanism, resulting in attention being cast toward areas that do not contribute to solving the task at hand.

 \vspace{-1em}

\begin{wraptable}{r}{2.75cm}
\vspace{-1em}
\hspace{-2.5em}
    \footnotesize
    \centering
    \begin{tabular}{lc}
    \toprule
    Prompt&Accuracy(\%)\\
    \midrule
    Baseline&49.3 \\
    \midrule
    CoT & 34.5 \\
    QVix &55.0\\
    \bottomrule
    \end{tabular}
       \vspace{-1em}
       \hspace{-2.5em}
    \caption{\footnotesize QVix vs. Zero-Shot CoT.}
    \label{tab:cot}
       \vspace{-1em}
\end{wraptable}

\paragraph{Comparison with Zero-Shot CoT.}
Here we compare QVix with zero-shot CoT~\cite{wei2022chain}. For  zero-shot CoT, we use the prompt \emph{``Let's think step by step by looking at the image.''} to generate rationale and then condition on the rationale to perform the final reasoning. We find that LVLM fails to generate reasonable rationales as the  CoT reasoning is usually regarded as an emergent ability but the open-source LVLM is usually built upon 10B-scale LLM which lacks CoT reasoning ability. As indicated in Table~\ref{tab:cot}, CoT's performance falls short, not only relative to QVix but also when compared to the baseline. In contrast, QVix actively steers the LVLM to scrutinize critical visual regions, thereby significantly bolstering the reasoning efficacy of open-source LVLMs.

\vspace{-1em}

\paragraph{Number of Pre-Questions.}
A key parameter in QVix is the number of pre-questions. Too few pre-questions may fail to provide sufficient contextual information, while an excess of pre-questions could render the model's reasoning overly challenging. 
\begin{wraptable}{r}{4cm}
\vspace{-1.em}
\hspace{-2.5em}
    \footnotesize
    \centering
    \begin{tabular}{lcc}
    \toprule
    Method&Number&Accuracy(\%)\\
    \midrule
    Baseline&-&49.3 \\
    \midrule
    \multirow{3}{*}{QVix}&2 & 51.1 \\
    &4 &55.0\\
    &6 &49.5\\
    \bottomrule
    \end{tabular}
       \vspace{-1em}
       \hspace{-2.5em}
     \caption{\footnotesize Number of pre-questions.}
     \label{tab:number}
        \vspace{-1em}
\end{wraptable}
We study the proper number of pre-questions in Table~\ref{tab:number}. 
When two pre-questions are used, there is a modest increase in accuracy to 51.1\%, suggesting that even a minimal addition of context can be beneficial.
However, the most notable improvement is observed when the number of pre-questions is increased to four, with accuracy peaking at 55.0\%. This finding implies that four pre-questions strike a delicate balance between providing adequate context for the model to process the task effectively and avoiding an information overload that could potentially confuse the model.
Interestingly, when the number of pre-questions is further increased to six, accuracy drops to 49.5\%, which is marginally higher than the baseline but lower than with two pre-questions.  This decrease may indicate that additional context does not translate into better performance but may hinder the model by introducing unnecessary complexity.


\vspace{-1em}

\paragraph{Prompt Stability.}
\begin{wraptable}{r}{4cm}
\vspace{-1.em}
\hspace{-2.8em}
    \footnotesize
    \centering
    \begin{tabular}{lcc}
    \toprule
    Method&Prompt&Accuracy(\%)\\
    \midrule
    Baseline&-&49.3 \\
    \midrule
    \multirow{3}{*}{QVix}&1 & 59.1 \\
    &2 &57.2\\
    &3 &57.1\\
    \bottomrule
    \end{tabular}
    \vspace{-1.em}
\hspace{-2.8em}
    \caption{Different Prompts.}
    \label{tab:stable}
    \vspace{-1em}
\end{wraptable}
In order to analyze the stability of our hand-written pre-question generation prompt, we employ GPT to rewrite our manually designed prompts in three different versions. The results are shown in Table~\ref{tab:stable}. This analysis indicates that while there may be slight fluctuations in outcomes with different prompt versions,
the QVix method contributes to stable and enhanced performance compared to the baseline. The ability of QVix to consistently outperform the baseline through various rewrites confirms its potential as a reliable and effective tool for improving the accuracy of vision-language tasks.








